Bayesian Optimization for Function-Valued Responses under Min-Max Criteria

Bayesian optimization is widely used for optimizing expensive black box functions, but most existing approaches focus on scalar responses. In many scientific and engineering settings the response is functional, varying smoothly over an index such as time or wavelength, which makes classical formulations inadequate. Existing methods often minimize integrated error, which captures average performance but neglects worst case deviations. To address this limitation we propose min-max Functional Bayesian Optimization (MM-FBO), a framework that directly minimizes the maximum error across the functional domain. Functional responses are represented using functional principal component analysis, and Gaussian process surrogates are constructed for the principal component scores. Building on this representation, MM-FBO introduces an integrated uncertainty acquisition function that balances exploitation of worst case expected error with exploration across the functional domain. We provide two theoretical guarantees: a discretization bound for the worst case objective, and a consistency result showing that as the surrogate becomes accurate and uncertainty vanishes, the acquisition converges to the true min-max objective. We validate the method through experiments on synthetic benchmarks and physics inspired case studies involving electromagnetic scattering by metaphotonic devices and vapor phase infiltration. Results show that MM-FBO consistently outperforms existing baselines and highlights the importance of explicitly modeling functional uncertainty in Bayesian optimization.

==> Figures/NM2.tex <==
\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Image [id:dp3872309002268697] 
\draw (320.5,149.3) node  {\includegraphics[width=270.75pt,height=203.25pt]{Figures/Noise.jpg}
};
% Text Node
\draw (146,10) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle \epsilon (a_j, e_j)$};
% Text Node
\draw (499,258) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle a_{i}$};
% Text Node
\draw (403,49) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle e_j \ =\ 0.8$};
% Text Node
\draw (325,130) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle e_j \ =\ 0.5$};
% Text Node
\draw (239,209) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle e_j \ =\ 0.2$};
% Text Node
\draw (227,136) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle e_j \ =\ 0.4$};
\end{tikzpicture}

==> Figures/noise_estimation.tex <==


\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Circle [id:dp16965915617398952] 
\draw  [fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=0.27 ] (98.56,110.78) .. controls (98.56,106.64) and (101.91,103.28) .. (106.06,103.28) .. controls (110.2,103.28) and (113.56,106.64) .. (113.56,110.78) .. controls (113.56,114.92) and (110.2,118.28) .. (106.06,118.28) .. controls (101.91,118.28) and (98.56,114.92) .. (98.56,110.78) -- cycle ;
%Rounded Rect [id:dp015370372061420445] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.4 ][line width=1.5]  (171.5,49.82) .. controls (171.5,44.77) and (175.6,40.67) .. (180.66,40.67) -- (271.34,40.67) .. controls (276.4,40.67) and (280.5,44.77) .. (280.5,49.82) -- (280.5,77.29) .. controls (280.5,82.35) and (276.4,86.44) .. (271.34,86.44) -- (180.66,86.44) .. controls (175.6,86.44) and (171.5,82.35) .. (171.5,77.29) -- cycle ;
%Straight Lines [id:da25110670761166376] 
\draw    (113.17,107.83) -- (169.58,64.22) ;
\draw [shift={(171.17,63)}, rotate = 142.3] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2657662055171923] 
\draw    (113.56,113.78) -- (168.7,164.64) ;
\draw [shift={(170.17,166)}, rotate = 222.69] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da2527620168217193] 
\draw [line width=0.75]    (280.5,63) -- (316.33,62.47) ;
\draw [shift={(318.33,62.44)}, rotate = 179.16] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da3070077252141077] 
\draw    (372.39,72.44) -- (372.39,143.78)(369.39,72.44) -- (369.39,143.78) ;
\draw [shift={(370.89,151.78)}, rotate = 270] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da09901437491300591] 
\draw    (440,162.83) -- (488.19,111.24) ;
\draw [shift={(489.56,109.78)}, rotate = 133.05] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Rounded Rect [id:dp2138266628847041] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=0.4 ][line width=1.5]  (170.5,149.82) .. controls (170.5,144.77) and (174.6,140.67) .. (179.66,140.67) -- (270.34,140.67) .. controls (275.4,140.67) and (279.5,144.77) .. (279.5,149.82) -- (279.5,177.29) .. controls (279.5,182.35) and (275.4,186.44) .. (270.34,186.44) -- (179.66,186.44) .. controls (174.6,186.44) and (170.5,182.35) .. (170.5,177.29) -- cycle ;
%Straight Lines [id:da8609366492831965] 
\draw    (279.5,164.67) -- (315.56,165.09) ;
\draw [shift={(317.56,165.11)}, rotate = 180.67] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;
%Straight Lines [id:da968242958014216] 
\draw    (440,162.83) -- (488.89,217.62) ;
\draw [shift={(490.22,219.11)}, rotate = 228.25] [color={rgb, 255:red, 0; green, 0; blue, 0 }  ][line width=0.75]    (10.93,-3.29) .. controls (6.95,-1.4) and (3.31,-0.3) .. (0,0) .. controls (3.31,0.3) and (6.95,1.4) .. (10.93,3.29)   ;

% Text Node
\draw (99.5,83.67) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle \textbf{e}$};
% Text Node
\draw (170,50.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\begin{minipage}[lt]{80pt}\setlength\topsep{0pt}
\begin{center}
\textbf{Expert labeler}\\\textbf{ (oracle)}
\end{center}

\end{minipage}};
% Text Node
\draw (201.83,157.67) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {\textbf{labeler}};

% Text Node
\draw (218.17,120.33) node [anchor=north west][inner sep=0.75pt]  [font=\small] [align=left] {$\displaystyle a$};
% Text Node
\draw (322.83,52.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle y$ (true label)};
% Text Node
\draw (323.17,154.33) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle \hat{y} \ ($estimated label)};
% Text Node
\draw (630,208.83) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle x=( e,a) ,\ z=1$};
% Text Node
\draw (630,102) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize] [align=left] {$\displaystyle x=( e ,a) ,\ z=0$};
% Text Node
\draw (495.67,210.17) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 65; green, 117; blue, 5 }  ,opacity=1 ] [align=left] {\textbf{{\footnotesize correct estimation:}}};
% Text Node
\draw (492.33,102.5) node [anchor=north west][inner sep=0.75pt]  [font=\footnotesize,color={rgb, 255:red, 208; green, 2; blue, 27 }  ,opacity=1 ] [align=left] {{\footnotesize \textbf{wrong estimation:}}};


\end{tikzpicture}


==> Figures/opt_assignment.tex <==
\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,300); %set diagram left start at 0, and has height of 300

%Shape: Circle [id:dp5296970761030637] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (171.33,63) .. controls (171.33,59.13) and (174.47,56) .. (178.33,56) .. controls (182.2,56) and (185.33,59.13) .. (185.33,63) .. controls (185.33,66.87) and (182.2,70) .. (178.33,70) .. controls (174.47,70) and (171.33,66.87) .. (171.33,63) -- cycle ;
%Shape: Circle [id:dp9966137922356793] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (211.33,63) .. controls (211.33,59.13) and (214.47,56) .. (218.33,56) .. controls (222.2,56) and (225.33,59.13) .. (225.33,63) .. controls (225.33,66.87) and (222.2,70) .. (218.33,70) .. controls (214.47,70) and (211.33,66.87) .. (211.33,63) -- cycle ;
%Shape: Circle [id:dp15565082703333588] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (326.33,63) .. controls (326.33,59.13) and (329.47,56) .. (333.33,56) .. controls (337.2,56) and (340.33,59.13) .. (340.33,63) .. controls (340.33,66.87) and (337.2,70) .. (333.33,70) .. controls (329.47,70) and (326.33,66.87) .. (326.33,63) -- cycle ;
%Shape: Triangle [id:dp9020418333762501] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (198.17,121) -- (207.33,140) -- (189,140) -- cycle ;
%Shape: Triangle [id:dp165383938470673] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (342.17,119) -- (351.33,138) -- (333,138) -- cycle ;
%Straight Lines [id:da1443298486911877] 
\draw    (178.33,70) -- (198.17,121) ;
%Straight Lines [id:da070280432799805] 
\draw    (218.33,70) -- (198.17,121) ;
%Straight Lines [id:da05229986825417332] 
\draw    (333.33,70) -- (342.17,119) ;
%Shape: Circle [id:dp9149327742514348] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (250.33,62) .. controls (250.33,58.13) and (253.47,55) .. (257.33,55) .. controls (261.2,55) and (264.33,58.13) .. (264.33,62) .. controls (264.33,65.87) and (261.2,69) .. (257.33,69) .. controls (253.47,69) and (250.33,65.87) .. (250.33,62) -- cycle ;
%Shape: Circle [id:dp16433558988889008] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (290.33,62) .. controls (290.33,58.13) and (293.47,55) .. (297.33,55) .. controls (301.2,55) and (304.33,58.13) .. (304.33,62) .. controls (304.33,65.87) and (301.2,69) .. (297.33,69) .. controls (293.47,69) and (290.33,65.87) .. (290.33,62) -- cycle ;
%Shape: Triangle [id:dp4358967168925587] 
\draw  [fill={rgb, 255:red, 74; green, 144; blue, 226 }  ,fill opacity=1 ] (277.17,120) -- (286.33,139) -- (268,139) -- cycle ;
%Straight Lines [id:da6456830356261345] 
\draw    (257.33,69) -- (277.17,120) ;
%Straight Lines [id:da3267495154726199] 
\draw    (297.33,69) -- (277.17,120) ;

% Text Node
\draw (171,36) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle e_{1}$};
% Text Node
\draw (212,35) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle e_{2}$};
% Text Node
\draw (250,34) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle e_{3}$};
% Text Node
\draw (291,33) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle e_{4}$};
% Text Node
\draw (326,33) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle e_{5}$};
% Text Node
\draw (191,143) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle a_{1}$};
% Text Node
\draw (270,142) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle a_{2}$};
% Text Node
\draw (335,141) node [anchor=north west][inner sep=0.75pt]   [align=left] {$\displaystyle a_{3}$};

\end{tikzpicture}
